Introduction to Arithmetic Groups

This book provides a gentle introduction to the study of arithmetic subgroups of semisimple Lie groups. This means that the goal is to understand the group SL(n,Z) and certain of its subgroups. Among the major results discussed in the later chapters are the Mostow Rigidity Theorem, the Margulis Superrigidity Theorem, Ratner's Theorems, and the classification of arithmetic subgroups of classical groups. As background for the proofs of these theorems, the book provides primers on lattice subgroups, arithmetic groups, real rank and Q-rank, ergodic theory, unitary representations, amenability, Kazhdan's property (T), and quasi-isometries. Numerous exercises enhance the book's usefulness both as a textbook for a second-year graduate course and for self-study. In addition, notes at the end of each chapter have suggestions for further reading. (Proofs in this book often consider only an illuminating special case.) Readers are expected to have some acquaintance with Lie groups, but appendices briefly review the prerequisite background.

==> Notation.tex <==
%!TEX root = IntroArithGrps.tex

\chapter*{List of Notation}

 \NotationIndex


==> Part6-BackMatter.tex <==
%!TEX root = IntroArithGrps.tex

\part*{Back Matter}


==> boxmatrix.tex <==

\def\boxmatrix#1{\setbox0=
 \vbox{\kern3pt\hbox{\kern3pt$\displaystyle
   \matrix{#1}$\kern3pt}\kern3pt}
 \dimen0=\wd0
 \divide \dimen0 by 4
 \lower\dimen0\vbox{\hrule\hbox to \wd0{\vrule\hss
      \vbox{\copy0}\hss\vrule}\hrule}}

\def\boxit#1{\setbox0=
 \vbox{\kern3pt\hbox{\kern3pt
 #1\kern3pt}\kern3pt}
  \dimen0=\ht0
 \divide \dimen0 by 2
 \hbox{\lower\dimen0\vbox{\hrule\hbox to \wd0{\vrule\hss
      \vbox{\copy0}\hss\vrule}\hrule}}}

% Example:
% $$\pmatrix{
%  \boxmatrix{0&1\cr -1&0 \cr} & 0 \cr
%   & \boxmatrix{
%  \cos \theta & \sin \theta \cr
%  -\sin \theta & \cos \theta \cr
%  -\sin \theta & \cos \theta \cr} \cr
%  }$$


==> thmlist.tex <==
%!TEX TS-program = makeindex


==> titlefont.tex <==
%% adapted from mem36.clo

\makeatletter

\renewcommand{\normalsize}{%
   \@setfontsize\normalsize{36}{45}% {36}{45}
   \abovedisplayskip 36\p@ \@plus8\p@ \@minus12\p@
   \abovedisplayshortskip \z@ \@plus8\p@
   \belowdisplayshortskip 22\p@ \@plus11\p@ \@minus5\p@
   \belowdisplayskip \abovedisplayskip
   \let\@listi\@listI}
\normalsize
\renewcommand{\small}{%
   \@setfontsize\small{30}{37}%
   \abovedisplayskip 30\p@ \@plus7\p@ \@minus11\p@
   \abovedisplayshortskip \z@ \@plus7\p@
   \belowdisplayshortskip 18\p@ \@plus9\p@ \@minus4\p@
   \def\@listi{\leftmargin\leftmargini
               \topsep 24\p@ \@plus8\p@ \@minus12\p@
               \parsep 12\p@ \@plus4\p@ \@minus6\p@
               \itemsep \parsep}%
   \belowdisplayskip \abovedisplayskip
}
\renewcommand{\footnotesize}{%
   \@setfontsize\footnotesize{25}{30}%
   \abovedisplayskip 25\p@ \@plus6\p@ \@minus10\p@
   \abovedisplayshortskip \z@ \@plus6\p@
   \belowdisplayshortskip 15\p@ \@plus7.5\p@ \@minus4\p@
   \def\@listi{\leftmargin\leftmargini
               \topsep 20\p@ \@plus7\p@ \@minus10\p@
               \parsep 10\p@ \@plus4\p@ \@minus5\p@
               \itemsep \parsep}%
   \belowdisplayskip \abovedisplayskip
}
%\renewcommand*{\miniscule}{\@setfontsize\miniscule{14}{17.5}
\renewcommand*{\tiny}{\@setfontsize\tiny{17}{22}}
\renewcommand*{\scriptsize}{\@setfontsize\scriptsize{20}{25}}
\renewcommand*{\large}{\@setfontsize\large{48}{60}}
\renewcommand*{\Large}{\@setfontsize\Large{50.75}{60}}
\renewcommand*{\LARGE}{\@setfontsize\LARGE{72}{86}}
\renewcommand*{\huge}{\@setfontsize\huge{84}{100}}
\renewcommand*{\Huge}{\@setfontsize\Huge{96}{116}}
%\renewcommand*{\HUGE}{\@setfontsize\HUGE{108}{132}
%\setlength{\onelineskip}{45\p@}
\if@twocolumn
  \setlength\parindent{1em}
\else
  \setlength\parindent{1.5em}
\fi
\setlength\smallskipamount{9\p@ \@plus2\p@ \@minus2\p@}
\setlength\medskipamount{18\p@ \@plus4\p@ \@minus4\p@}
\setlength\bigskipamount{36\p@ \@plus8\p@ \@minus8\p@}
\setlength\headheight{45\p@}
\setlength\headsep{65\p@}
\setlength\topskip{36\p@}
\setlength\footskip{90\p@}
\setlength\maxdepth{.5\topskip}
\setlength\@maxdepth\maxdepth
\setlength\footnotesep{21\p@}
\setlength{\skip\footins}{35\p@ \@plus 12\p@ \@minus 6\p@}
\setlength\floatsep    {36\p@ \@plus 8\p@ \@minus 8\p@}
\setlength\textfloatsep{65\p@ \@plus 8\p@ \@minus 16\p@}
\intextsep \floatsep
\dblfloatsep \floatsep
\dbltextfloatsep \textfloatsep
\setlength\@fptop{0\p@ \@plus 1fil}
\setlength\@fpsep{31\p@ \@plus 2fil}
\@fpbot \@fptop
\@dblfptop \@fptop
\@dblfpsep \@fpsep
\@dblfpbot \@dblfptop
%\setlength\lxvchars{891\p@} %
%\setlength\xlvchars{617\p@} %
\if@twocolumn
  \setlength\marginparsep{1em}
\else
  \setlength\marginparsep{0.7em}
\fi
  \setlength\marginparpush{0.5em}

\makeatother
